TMPO: Trajectory Matching Policy Optimization for Diverse and Efficient Diffusion Alignment

Reinforcement learning (RL) has shown extraordinary potential in aligning diffusion models to downstream tasks, yet most of them still suffer from significant reward hacking, which degrades generative diversity and quality by inducing visual mode collapse and amplifying unreliable rewards. We identify the root cause as the mode-seeking nature of these methods, which maximize expected reward without effectively constraining probability distribution over acceptable trajectories, causing concentration on a few high-reward paths. In contrast, we propose Trajectory Matching Policy Optimization (TMPO), which replaces scalar reward maximization with trajectory-level reward distribution matching. Specifically, TMPO introduces a Softmax Trajectory Balance (Softmax-TB) objective to match the policy probabilities of K trajectories to a reward-induced Boltzmann distribution. We prove that this objective inherits the mode-covering property of forward KL divergence, preserving coverage over all acceptable trajectories while optimizing reward. To further reduce multi-trajectory training time on large-scale flow-matching models, TMPO incorporates Dynamic Stochastic Tree Sampling, where trajectories share denoising prefixes and branch at dynamically scheduled steps, reducing redundant computation while improving training effectiveness. Extensive results across diverse alignment tasks such as human preference, compositional generation and text rendering show that TMPO improves generative diversity over state-of-the-art methods by 9.1%, and achieves competitive performance in all downstream and efficiency metrics, attaining the optimal trade-off between reward and diversity.

==> NeurIPS_2026_TMPO__Preprint_/checklist.tex <==
\section*{NeurIPS Paper Checklist}



\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    \item[] Justification: The abstract and introduction clearly state three contributions: (i)~reformulating visual alignment as trajectory-level reward distribution matching, (ii)~deriving the Softmax-TB objective with a formal mode-covering guarantee (Section~\ref{prop:mode_covering}), and (iii)~introducing a dynamic prefix-sharing tree sampler. All claims are supported by theoretical analysis (Section~\ref{headings} and Appendix~\ref{appendix:theoretical_derivations}) and experimental evaluation (Section~\ref{sec:experiments}). Limitations are discussed in the Conclusion.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A \answerNo{} or \answerNA{} answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    \item[] Justification: The Conclusion includes a dedicated ``Limitations \& Future Work'' paragraph that discusses two limitations: (1)~the Boltzmann target quality is upper-bounded by the underlying reward model, and (2)~evaluation is restricted to text-to-image generation, with extensions to video, 3D, and robotic generation left as future work.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate ``Limitations'' section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{}
    \item[] Justification: The mode-covering equilibrium result (Section~\ref{prop:mode_covering}) is stated with explicit assumptions and proved in the main text; an extended proof with all intermediate steps is provided in Appendix~\ref{appendix:forward_kl}. The max-entropy derivation of the Boltzmann target, partition function elimination, gradient direction analysis, and mode-covering vs.\ mode-seeking characterization are all formally derived in Appendix~\ref{appendix:theoretical_derivations}. The IS ratio decomposition and bias correction are derived in Appendix~\ref{appendix:gradient_analysis}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}
    \item[] Justification: Section~\ref{sec:experiments} describes the evaluation protocol, metrics, and baselines. Appendix~\ref{app:sec:exp-setup-details} provides full hyperparameter specifications (Section~\ref{app:subsubsec:synthetic-hyperp}), the complete training pipeline, model sources with URLs (Table~\ref{tab:model_links}), LoRA configuration, reward normalization details, and compute resources (Section~\ref{app:subsubsec:synthetic-compute}).
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item If the paper includes experiments, a \answerNo{} answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and\slash or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{}
    \item[] Justification: Anonymized source code is provided in the abstract (\url{https://anonymous.4open.science/r/TMPO-2E2B}) and will also be included in the supplementary material. Full code and trained model checkpoints will be publicly released upon publication. Training prompts for the human-preference protocol are drawn from the publicly available HPDv2 dataset; the GenEval and OCR protocols use task-specific prompt sets. All backbone and reward models used are publicly accessible; URLs are provided in Table~\ref{tab:model_links}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so \answerNo{} is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerYes{}
    \item[] Justification: Section~\ref{sec:experiments} specifies the backbone model, LoRA configuration, image resolution, evaluation protocol (10 images per prompt), and all baselines. Appendix~\ref{app:subsubsec:synthetic-hyperp} provides complete hyperparameter tables covering optimizer, learning rate, scheduling, clipping, $\beta$ warmup, tree sampling parameters, and EMA configuration for all three training protocols.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{}
    \item[] Justification: Due to the high computational cost of training large-scale flow models (each run requires 42--204 GPU-hours on 8 GPUs depending on protocol, i.e., 5.3--25.5 wall-clock hours; details in Appendix~\ref{app:subsubsec:synthetic-compute}), we do not report error bars from multiple independent runs. However, evaluation is conducted over a held-out prompt set with 10 independent samples per prompt, and we report multiple complementary metrics (HPS-v2.1, ImageReward, PickScore, LGMD) to provide a comprehensive assessment.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g., negative error rates).
        \item If error bars are reported in tables or plots, the authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: Appendix~\ref{app:subsubsec:synthetic-compute} specifies the hardware (8 GPUs), distributed training framework (FSDP via HuggingFace Accelerate), precision (bf16), and total GPU-hours per run. Per-iteration wall-clock times are reported in all main result tables.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}
    \item[] Justification: We have reviewed the NeurIPS Code of Ethics and confirm that the research conforms to it. Our work uses publicly available models and datasets, and does not involve human subjects or private data.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer \answerNo, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{}
    \item[] Justification: This work is foundational and algorithmic: it proposes a new training objective (Softmax Trajectory Balance) and a sampling scheme (Dynamic Stochastic Tree Sampling) for fine-tuning an existing publicly released text-to-image backbone (FLUX.1-dev). It does not introduce new generative capabilities, datasets, or application domains beyond the base model, and there is no direct path from the contribution itself to specific deployments or downstream applications. Any societal implications are inherited from the underlying base model and the existing diffusion-alignment paradigm rather than introduced by this paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that there is no societal impact of the work performed.
        \item If the authors answer \answerNA{} or \answerNo, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate Deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}
    \item[] Justification: TMPO fine-tunes an existing publicly available model (FLUX.1-dev) using LoRA adapters with publicly available reward models. The trained LoRA weights do not introduce new generative capabilities beyond those of the base model; they only adjust the probability distribution over existing generation modes. We do not release a new foundation model or scraped dataset.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}
    \item[] Justification: All models and datasets used are properly cited. Table~\ref{tab:model_links} provides URLs and references for the backbone (FLUX.1-dev, released under the FLUX.1-dev Non-Commercial License) and all reward models (HPS-v2.1 under Apache License 2.0, ImageReward under MIT License, PickScore under MIT License). The HPDv2 prompt dataset (CC-BY-NC 4.0) is cited in the main text. All assets are used in accordance with their respective licenses for non-commercial academic research.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper does not introduce new datasets or pre-trained models as standalone assets. Code will be released upon publication with documentation.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset\slash code\slash model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{}
    \item[] Justification: This paper does not involve crowdsourcing or research with human subjects. All evaluations use automatic reward models.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}
    \item[] Justification: This paper does not involve research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNA{}
    \item[] Justification: LLMs are not used as a component of the core methodology in this research.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy in the NeurIPS handbook for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> NeurIPS_2026_TMPO__Preprint_/sections/abstract.tex <==
Reinforcement learning (RL) has shown extraordinary potential in aligning diffusion models to downstream tasks, yet most of them still suffer from significant reward hacking, which degrades generative diversity and quality by inducing visual mode collapse and amplifying unreliable rewards. We identify the root cause as the \textit{mode-seeking} nature of these methods, which maximize expected reward without effectively constraining probability distribution over acceptable trajectories, causing concentration on a few high-reward paths. In contrast, we propose \textbf{Trajectory Matching Policy Optimization (TMPO)}, which replaces scalar reward maximization with trajectory-level reward distribution matching. Specifically, TMPO introduces a \textbf{Softmax Trajectory Balance (Softmax-TB)} objective to match the policy probabilities of $K$ trajectories to a reward-induced Boltzmann distribution. We prove that this objective inherits the \textit{mode-covering} property of forward KL divergence, preserving coverage over all acceptable trajectories while optimizing reward. To further reduce multi-trajectory training time on large-scale flow-matching models, TMPO incorporates \textbf{Dynamic Stochastic Tree Sampling}, where trajectories share denoising prefixes and branch at dynamically scheduled steps, reducing redundant computation while improving training effectiveness. Extensive results across diverse alignment tasks such as human preference, compositional generation and text rendering show that TMPO improves generative diversity over state-of-the-art methods by 9.1\%, and achieves competitive performance in all downstream and efficiency metrics, attaining the optimal trade-off between reward and diversity.


==> NeurIPS_2026_TMPO__Preprint_/sections/abstract_zh.tex <==
% 中文翻译版 abstract（基于 sections/abstract.tex）
\begin{abstract}
强化学习（RL）在将扩散模型对齐到下游任务方面展现出巨大潜力，但现有方法常受奖励黑客影响，导致模式崩塌和生成多样性下降。我们将其根本原因归结为这些方法的\textit{模式寻求}本质——它们最大化期望奖励，却未能有效约束概率质量在可接受轨迹上的分配，导致概率集中于少数高奖励路径。为此，我们提出\textbf{轨迹匹配策略优化（TMPO）}，以轨迹级奖励分布匹配替代标量奖励最大化。具体而言，TMPO 引入\textbf{Softmax 轨迹平衡（Softmax-TB）}目标，将 $K$ 条轨迹的策略概率与奖励诱导的 Boltzmann 分布进行匹配。我们证明该目标继承了前向 KL 散度的\textit{模式覆盖}性质，在优化奖励的同时保持对可接受轨迹的概率覆盖。为进一步降低大规模流匹配模型上的多轨迹训练时间，TMPO 引入\textbf{动态随机树采样}，多条轨迹共享去噪前缀并在动态调度的步骤处分支，减少冗余计算的同时提升训练效果。在人类偏好、组合生成和文字渲染等多种对齐任务上的大量实验表明，TMPO 将生成多样性相比当前最优方法提升了 9.1\%，并在所有下游任务和效率指标上取得了competitive的表现，实现了奖励与多样性的最佳权衡。
\end{abstract}


==> NeurIPS_2026_TMPO__Preprint_/sections/conclusion.tex <==
\section{Conclusion}
We presented TMPO, which reformulates diffusion RL alignment as trajectory-level distribution matching via Softmax Trajectory Balance, a partition-free objective whose advantage characterizes the forward KL divergence, inheriting mode-covering diversity guarantees without auxiliary regularization. Combined with prefix-sharing tree rollouts and dynamic branching, TMPO achieves the best reward--diversity trade-off across all evaluated settings while reducing iteration time by up to 27\%.

\paragraph{Limitations \& Future Work.}
This work focuses on T2I alignment; two natural extensions are:
(1)~the Boltzmann target quality is upper-bounded by the underlying reward model; pairing TMPO with stronger reward models may yield further improvements, and
(2)~extending trajectory-level distribution matching to video generation, 3D synthesis, and robotic action generation.


==> NeurIPS_2026_TMPO__Preprint_/sections/experiments.tex <==
\section{Experiments}
\label{sec:experiments}

This section empirically evaluates TMPO on three tasks: (1) Compositional Image Generation, (2) Visual Text Rendering, and (3) Human Preference Alignment. Beyond alignment quality, we also assess generative diversity and per-iteration training efficiency.

\subsection{Experimental setup}

\paragraph{Models, prompts, and metrics.}
We use FLUX.1-dev as the backbone, fine-tuned with LoRA~\cite{hu2022lora} (rank $r{=}64$, $\alpha{=}128$) targeting all attention and feed-forward projections in each transformer block. All images are generated at $512{\times}512$ resolution. Training rollouts use $6$ denoising steps for efficiency; all evaluations use $28$ steps. For human preference alignment, training and evaluation prompts are drawn from HPDv2~\cite{wu2023hpsv2}. For compositional image generation (GenEval) and visual text rendering (OCR), we construct task-specific training and test prompt sets. All evaluations generate 10 images per prompt. Task-specific metrics include GenEval~\cite{ghosh2024geneval} accuracy for composition, OCR accuracy ($1{-}\text{NED}$) for text rendering, and HPS-v2.1, ImageReward, PickScore for preference alignment. Diversity is measured by two complementary metrics. \textbf{Log Geometric Mean Distance (LGMD)} computes the log geometric mean of pairwise distances in VAE~\cite{kingma2014auto} latent space: $\text{LGMD} = \frac{2}{N(N{-}1)} \sum_{i<j} \log \bigl(\|\phi(x_i) - \phi(x_j)\|_2 / \sqrt{D}\bigr)$, where $\phi(\cdot)$ is the flattened VAE latent and $D$ the feature dimension; positive values indicate healthy diversity, while negative values signal mode collapse. \textbf{Cosine Diversity (Cos.\,Div.)} follows GARDO~\cite{he2025gardo} and measures the mean pairwise cosine distance in DINOv2~\cite{oquab2024dinov2} ViT-L/14 feature space: $\text{Cos.\,Div.} = \frac{2}{N(N{-}1)}\sum_{i<j}(1 - \cos(\psi(x_i), \psi(x_j)))$. LGMD captures low-level structural duplicates, while Cos.\,Div.\ captures semantic layout and texture differences.

\paragraph{Training protocols and baselines.}
We consider three single-reward protocols, namely GenEval only (compositional accuracy), OCR only (text rendering accuracy), and PickScore~\cite{kirstain2023pick} only (human preference), as well as joint preference training with HPS-v2.1, ImageReward, and PickScore at equal weight, where each reward is independently z-score normalized within the $K$-trajectory group before summation. TMPO uses a three-level prefix-sharing tree with $K{=}3^3{=}27$ terminal trajectories per prompt. TMPO is compared against Flow-GRPO~\cite{liu2025flowgrpo}, MixGRPO~\cite{li2025mixgrpo}, TreeGRPO~\cite{ding2026treegrpo}, and GARDO~\cite{he2025gardo} under matched backbone and reward settings. All GRPO-based baselines adopt KL regularization with $\beta_{\text{KL}}{=}0.03$. Full hyperparameter specifications, model details, and compute resources are provided in Appendix~\ref{app:sec:exp-setup-details}.

\subsection{Main results}

Table~\ref{tab:main_results} summarizes results across three training protocols. Joint multi-reward results are provided in Table~\ref{tab:comparison_joint} (Appendix~\ref{app:sec:extended-exp-results}). TMPO also generalizes to SD3.5-Medium, outperforming all baselines under the PickScore only protocol (Table~\ref{tab:sd35} in Appendix~\ref{app:subsec:sd35}).

\begin{figure*}[h]
    \centering
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/Time_Geneval.pdf}
        \caption{\textbf{GenEval (composition)}}
        \label{fig:training_step_geneval}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/Time_OCR.pdf}
        \caption{\textbf{OCR Acc.\ (text rendering)}}
        \label{fig:training_step_ocr}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/Time_Pick.pdf}
        \caption{\textbf{PickScore (preference)}}
        \label{fig:training_steps_pickscore}
    \end{subfigure}
    \caption{\textbf{Training curves across three single-reward protocols.} Each plot shows the task reward versus wall-clock training time. TMPO converges faster and reaches higher final reward than all baselines, benefiting from both prefix-sharing tree sampling and Softmax-TB distribution matching.}
    \label{fig:training_curves}
\end{figure*}

\paragraph{Compositional image generation.}
Under GenEval only training, TMPO achieves the best compositional accuracy (0.949) while preserving superior diversity on both LGMD and Cosine Diversity. Despite the sparse binary reward signal, Softmax-TB effectively distributes probability mass toward compositionally correct trajectories without collapsing onto a narrow set of solutions.

\paragraph{Visual text rendering.}
TMPO achieves the best iteration time, the highest HPS-v2.1 and PickScore, and the best diversity on both LGMD and Cosine Diversity. Although Flow-GRPO reaches the highest OCR accuracy, it substantially reduces diversity, indicating stronger overfitting to the task reward.

\paragraph{Human preference alignment.}
Under PickScore only training, TMPO obtains the best PickScore and diversity, with competitive HPS-v2.1 and ImageReward. Under joint training (Table~\ref{tab:comparison_joint}), TMPO again achieves the best HPS-v2.1 and LGMD, confirming that distribution matching transfers better across unseen preference metrics. Figure~\ref{fig:training_curves} shows training curves across all three protocols; qualitative examples are shown in Figure~\ref{fig:demo}.

\begin{table}[h]
  \centering
  \caption{Performance on Compositional Image Generation, Visual Text Rendering, and Human Preference benchmarks on FLUX.1-dev, evaluated by task performance on task-specific test prompts and by preference scores and diversity on DrawBench prompts. Best values are \textbf{bold} and second-best are \underline{underlined}. \colorbox{gray!10}{Light gray rows} denote the pretrained baseline without RL training. \colorbox{gray!20}{Dark gray rows} denote our approach. \colorbox{proxyorange!18}{Orange cells} mark the proxy reward used for training in each section. ImgRwd: ImageReward; Cos.\,Div.: DINOv2-space cosine diversity.}
  \label{tab:main_results}
  \resizebox{\columnwidth}{!}{
    \begin{tabular}{lcccccccc}
      \toprule
      \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Time (s)} $\downarrow$} & \multicolumn{2}{c}{\textbf{Task Metric} $\uparrow$} & \multicolumn{3}{c}{\textbf{Human Preference} $\uparrow$} & \multicolumn{2}{c}{\textbf{Diversity} $\uparrow$} \\
      \cmidrule(lr){3-4} \cmidrule(lr){5-7} \cmidrule(lr){8-9}
      & & \textbf{GenEval} & \textbf{OCR Acc.} & \textbf{HPS-v2.1} & \textbf{ImgRwd} & \textbf{PickScore} & \textbf{LGMD} & \textbf{Cos.\,Div.} \\
      \midrule
      \multicolumn{9}{c}{\textit{Compositional Image Generation}} \\
      \midrule
      \rowcolor{gray!10} FLUX.1-dev & --- & \cellcolor{proxyorange!18} 0.647 & --- & 0.301 & \underline{1.099} & \underline{22.301} & -0.031 & 0.211 \\
      Flow-GRPO & 160.7 & \cellcolor{proxyorange!18} \underline{0.943} & --- & 0.285 & 1.078 & 22.097 & -0.092 & 0.201 \\
      MixGRPO & 150.8 & \cellcolor{proxyorange!18} 0.932 & --- & \textbf{0.310} & 1.086 & 21.850 & -0.271 & 0.183 \\
      TreeGRPO & \underline{125.9} & \cellcolor{proxyorange!18} 0.939 & --- & 0.278 & 1.079 & 21.540 & -0.285 & 0.181 \\
      GARDO & 165.3 & \cellcolor{proxyorange!18} 0.923 & --- & 0.289 & 1.091 & 22.245 & \underline{0.012} & \underline{0.238} \\
      \rowcolor{gray!20}
      \textbf{TMPO (Ours)} & \textbf{91.9} & \cellcolor{proxyorange!18} \textbf{0.949} & --- & \underline{0.306} & \textbf{1.159} & \textbf{22.901} & \textbf{0.131} & \textbf{0.247} \\
      \midrule
      \multicolumn{9}{c}{\textit{Visual Text Rendering}} \\
      \midrule
      \rowcolor{gray!10} FLUX.1-dev & --- & --- & \cellcolor{proxyorange!18} 0.591 & \underline{0.292} & \textbf{1.121} & 21.968 & -0.040 & 0.215 \\
      Flow-GRPO & 121.3 & --- & \cellcolor{proxyorange!18} \textbf{0.940} & 0.291 & 1.100 & 21.365 & -0.092 & 0.208 \\
      MixGRPO & 116.2 & --- & \cellcolor{proxyorange!18} 0.919 & 0.282 & 1.098 & 20.878 & -0.302 & 0.179 \\
      TreeGRPO & \underline{93.4} & --- & \cellcolor{proxyorange!18} 0.921 & 0.290 & 1.110 & 21.099 & -0.292 & 0.180 \\
      GARDO & 123.8 & --- & \cellcolor{proxyorange!18} 0.931 & 0.291 & 1.085 & \underline{22.087} & \underline{0.064} & \underline{0.228} \\
      \rowcolor{gray!20}
      \textbf{TMPO (Ours)} & \textbf{76.3} & --- & \cellcolor{proxyorange!18} \underline{0.935} & \textbf{0.310} & \underline{1.111} & \textbf{22.309} & \textbf{0.110} & \textbf{0.241} \\
      \midrule
      \multicolumn{9}{c}{\textit{Human Preference Alignment}} \\
      \midrule
      \rowcolor{gray!10} FLUX.1-dev & --- & --- & --- & 0.310 & 1.119 & \cellcolor{proxyorange!18} 22.604 & \underline{-0.056} & \underline{0.214} \\
      Flow-GRPO & 108.9 & --- & --- & \textbf{0.377} & 1.600 & \cellcolor{proxyorange!18} \underline{24.210} & -0.107 & 0.209 \\
      MixGRPO & 103.5 & --- & --- & 0.367 & \textbf{1.621} & \cellcolor{proxyorange!18} 23.934 & -0.232 & 0.183 \\
      TreeGRPO & \underline{79.1} & --- & --- & 0.369 & 1.580 & \cellcolor{proxyorange!18} 23.657 & -0.284 & 0.176 \\
      GARDO & 112.7 & --- & --- & 0.343 & 1.571 & \cellcolor{proxyorange!18} 23.959 & -0.060 & 0.212 \\
      \rowcolor{gray!20}
      \textbf{TMPO (Ours)} & \textbf{68.3} & --- & --- & \underline{0.373} & \underline{1.610} & \cellcolor{proxyorange!18} \textbf{24.277} & \textbf{0.204} & \textbf{0.252} \\
      \bottomrule
    \end{tabular}
  }
\end{table}

\begin{figure*}[h]
  \centering
  \includegraphics[width=\textwidth]{figures/main_text_comparison.pdf}
  \caption{\textbf{Qualitative results of different alignment methods.} TMPO produces diverse, high-fidelity images that faithfully follow the text prompt.}
  \label{fig:demo}
\end{figure*}

\paragraph{Efficiency and diversity.}
TMPO improves the Pareto frontier between alignment, diversity, and training cost. Because trajectory log-probabilities accumulate only over $T{=}3$ stochastic branch points, gradient back-propagation is confined to these transitions rather than the full denoising horizon; combined with prefix sharing that amortizes forward computation, TMPO reduces iteration time by $\sim$20\% relative to TreeGRPO across three single-reward settings (Table~\ref{tab:main_results}; joint training in Table~\ref{tab:comparison_joint}). More importantly, the LGMD gap is consistent across all settings: GRPO-style baselines often raise reward scores while driving LGMD negative, whereas TMPO keeps LGMD positive in every setting.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.48\linewidth]{figures/TMPO-reward-diversity.pdf}
    \hfill
    \includegraphics[width=0.48\linewidth]{figures/TMPO-efficiency.pdf}
    \caption{\textbf{Pareto analysis of TMPO against GRPO-based alignment methods.} \textbf{Left:} normalized reward score versus generation diversity measured by LGMD. \textbf{Right:} normalized reward score versus iteration time. Normalized scores are computed via min-max normalization across all compared methods for each metric. TMPO achieves the most favorable trade-off in both reward-diversity and reward-efficiency comparisons.}
    \label{fig:pareto}
\end{figure}

\subsection{Ablation study}

We ablate major components of TMPO under the PickScore only protocol (Table~\ref{tab:ablation}), covering three categories: \textit{objective} (reward temperature $\beta$), \textit{balance granularity} (trajectory vs.\ step-wise), and \textit{sampling strategy} (tree structure, dynamic branching).

\begin{table}[hbt]
  \caption{Ablation study on FLUX.1-dev under the PickScore only protocol. Time denotes iteration time in seconds.}
  \label{tab:ablation}
  \centering
  \resizebox{\linewidth}{!}{%
  \begin{tabular}{lcccccc}
      \toprule
      \textbf{Variant} & \textbf{Time} $\downarrow$ & \textbf{HPS-v2.1} $\uparrow$ & \textbf{ImageReward} $\uparrow$ & \textbf{PickScore} $\uparrow$ & \textbf{LGMD} $\uparrow$ & \textbf{Cos.\,Div.} $\uparrow$ \\
      \midrule
      \textbf{TMPO (Full)} & \textbf{68.3} & \textbf{0.373} & \textbf{1.610} & \textbf{24.277} & \textbf{0.204} & \textbf{0.252} \\
      \midrule
      w/o Reward Temp.\ $\beta$ ($\beta{=}1$) & \underline{68.5} & 0.352 & 1.501 & 23.891 & \underline{0.199} & \underline{0.250} \\
      Step-wise Balance (Detailed) & 87.2 & 0.339 & 1.139 & 23.107 & 0.012 & 0.223 \\
      w/o Tree Structure ($K{=}27$) & 123.7 & \underline{0.369} & \underline{1.598} & \underline{24.109} & 0.173 & 0.245 \\
      w/o Dynamic Branching & 78.7 & 0.361 & 1.553 & 23.878 & 0.121 & 0.239 \\
      \bottomrule
    \end{tabular}%
  }
\end{table}

The results confirm the contribution of each component.
\textbf{w/o Reward Temp.\ $\beta$} removes the $\beta$-warmup schedule and fixes $\beta{=}1$ throughout training. Without progressive sharpening, the target distribution remains flat, slowing reward improvement (PickScore $24.28 \to 23.89$); however, the mild optimization pressure preserves diversity well (LGMD $0.199$, Cos.\,Div.\ $0.250$).
\textbf{Step-wise detailed balance} enforces per-step flow matching, causing severe loss oscillation and convergence difficulty. The substantial drop in ImageReward ($1.61 \to 1.14$) and near-zero LGMD ($0.012$) show that local supervision fragments credit assignment across the trajectory.
\textbf{w/o Tree Structure} uses $K{=}27$ independent rollouts and achieves comparable alignment, confirming the generality of Softmax-TB; however, iteration time increases by $81\%$ due to the loss of prefix sharing.
\textbf{w/o Dynamic Branching} fixes branch positions throughout training, resulting in lower diversity ($\Delta\text{LGMD} = -0.083$, $\Delta\text{Cos.\,Div.} = -0.013$) and higher iteration time ($78.7$\,s vs.~$68.3$\,s).


==> NeurIPS_2026_TMPO__Preprint_/sections/introduction.tex <==
\section{Introduction}

\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]{figures/toy_experiment_narrow.pdf}
    \caption{\textbf{A toy experiment on a three-layer MLP diffusion model pre-trained on a Gaussian mixture distribution containing non-reward modes and rare density modes.} The post-training objective is to match a multimodal reward distribution. GRPO-based reward maximization collapses to a single high-reward mode even with KL regularization, whereas TMPO covers all reward clusters by matching trajectory-level reward distributions while maintaining a high average reward.}
    \label{fig:toy_experiment}
    % \vspace{-1.5em}
\end{figure}

Recently, RL has achieved remarkable success in aligning Large Language Models (LLMs), generative diffusion models and flow-matching models. However, existing methods still suffer from significant \textit{reward hacking} issue, which implies the model may ignore the distribution diversity and instead take a shortcut by over-reinforcing a small proportion of the recognized high-reward modes. Similar to LLM, this dilemma can be called \textit{visual mode collapse}. While mitigating reward hacking has been extensively studied in the field of LLMs~\cite{moskovitz2023confronting,coste2023reward}, the issue remains largely unexplored for diffusion or flow models, which raises two critical issues: \emph{\textbf{1) Degradation of Diversity:}} for language models, a problem may solely own a single definite answer, whereas for generative models (\emph{i.e.,} text-to-image models), the same prompt may correspond to many plausible outputs that vary in \emph{composition}, \emph{spatial layout}, and \emph{scene semantics}. Reward hacking, however, drives the model to generate images with only a small set of compositions and styles, degrading generative diversity. (Fig.~\ref{fig:comparison}). \emph{\textbf{2) Amplification of Unreliable Rewards:}} for text-to-image models, both model-based rewards (\emph{e.g.,} ImageReward~\cite{xu2023imagereward}, HPS~\cite{wu2023hpsv2}, PickScore~\cite{kirstain2023pick}) and rule-based rewards (\emph{e.g.,} OCR accuracy and GenEval~\cite{ghosh2024geneval}) are intrinsically imperfect proxies for human preferences~\cite{gao2023scaling,chen2023textdiffuser,pan2022the,skalse2022defining,he2025gardo}. Reward hacking on these proxy rewards amplifies spuriously rewarded image attributes, thereby deteriorating generation quality. This raises a core question in generative diffusion alignment: \emph{How can we preserve the anisotropic distribution of outputs learned by the model from pre-training data while encouraging the model to satisfy rewards with specific preferences?}

% \researchquestion{How can we preserve the anisotropic distribution of outputs learned by the model from pre-training data while encouraging the model to satisfy rewards with specific preferences?}

The reward hacking behavior in diffusion model alignment can be attributed to the training objectives of current diffusion-based RL methods. Existing methods use reward maximization as the optimization objective~\cite{DDPO,fan2023dpok,liu2025flowgrpo,xue2025dancegrpo,li2025mixgrpo,ding2026treegrpo}, which we prove is intrinsically \textit{mode-seeking}. In particular, mode-seeking models tend to explore high-reward trajectory, rather than covering all reasonable counterparts, as illustrated by the GRPO example in Fig.~\ref{fig:toy_experiment}. \textbf{An ideal optimization objective should be \textit{mode-covering}, which encourages the model to cover as many reasonable solutions as possible.} This analysis further suggests that alleviating reward hacking requires a fundamental shift in the optimization objective. Existing methods mainly attempt to address the issue of reward hacking through two lines of work: \emph{\textbf{1) Constraining Over-optimization:}} KL regularization~\cite{ouyang2022training,stiennon2020learning,fan2023dpok,liu2025flowgrpo,he2025gardo} is used to constrain the deviation of the policy from the reference model, but it does not alter the reward-maximization objective, resulting in limited improvement in generative diversity. \emph{\textbf{2) Improving Training Objective:}} Generative Flow Network (GFlowNet)-based methods~\cite{zhang2024dgfs,zhang2025improving,liu2025nablagfn} seek to generate outputs with probabilities proportional to their rewards, but existing methods usually establish local constraints on individual denoising steps, which requires estimating an intractable state-flow function for policy updates, thereby introducing additional training error. Overall, existing mitigation methods still fall short of providing a direct mode-covering objective over the full denoising trajectory.

To address this gap, we propose \textbf{Trajectory Matching Policy Optimization (TMPO)}. Inspired by the reward distribution matching nature of GFlowNets~\cite{bengio2021flow}, TMPO fundamentally shifts the training objective from reward maximization to trajectory-level reward distribution matching. We prove that TMPO is \textit{mode-covering} and can naturally encourage the coverage of reasonable solutions, thereby alleviating reward hacking from the ground up, as shown in Fig.~\ref{fig:toy_experiment}. Specifically, we introduce a \textbf{Softmax Trajectory Balance (Softmax-TB)} objective, which performs reward distribution matching on the complete denoising trajectory. For $K$ trajectories generated from the same starting point, Softmax-TB matches the generation probabilities of these trajectories to a target Boltzmann distribution computed from rewards ( $P_\theta(\tau) \propto \exp(\beta R(\tau))$ ). Meanwhile, by normalizing the trajectory probabilities $P_\theta(\tau)$ and exponential rewards $\exp(\beta R(\tau))$ among the $K$ trajectories within each group, we eliminate the intractable partition function, yielding a simpler and directly optimizable objective. To reduce the training time of fully sampling multiple trajectories under Softmax-TB~\cite{zhang2025improving}, TMPO further introduces \textbf{Dynamic Stochastic Tree Sampling}~\cite{li2025mixgrpo,fu2025dynamictreerpo,ding2026treegrpo}, which allows trajectories to share denoising steps through a tree structure, reducing redundant computation and lowering training time. By dynamically adjusting the branching points, the tree sampler also promotes effective exploration at different denoising stages and improves training performance.

We evaluate TMPO on FLUX.1-dev across three alignment tasks: compositional image generation, visual text rendering, and human preference alignment. Results show that TMPO obtains the highest diversity metrics across all tasks, improving generative diversity by 9.1\% on average over existing state-of-the-art methods, while also achieving the best GenEval accuracy and PickScore. Moreover, TMPO reduces training time by up to 27\% compared with state-of-the-art methods and achieves the most favorable trade-offs in both reward-diversity and reward-efficiency comparisons, as shown in Fig.~\ref{fig:pareto}.

Our contributions are as follows: \textbf{(1)} We identify reward maximization as the root cause of reward hacking in diffusion-based RL and reformulate the optimization objective as reward distribution matching. \textbf{(2)} We introduce \textbf{Softmax Trajectory Balance}, a partition-function-free trajectory-level distribution matching objective, and prove that its mode-covering property naturally preserves generative diversity. \textbf{(3)} We introduce \textbf{Dynamic Stochastic Tree Sampling}, which substantially reduces the training time of our trajectory balance objective and enables scalable training on large-scale flow-matching models.


==> NeurIPS_2026_TMPO__Preprint_/sections/introduction_zh.tex <==
% 中文翻译版 introduction（基于 sections/introduction.tex）

\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]{figures/toy_experiment_narrow.pdf}
    \caption{在一个三层 MLP 扩散模型上的玩具实验，该模型在包含非奖励模式和稀有密度模式的高斯混合分布上预训练。后训练目标是匹配多模态奖励分布。基于 GRPO 的奖励最大化方法即使在 KL 正则化下仍坍缩到单一高奖励模式，而 TMPO 通过匹配轨迹级奖励覆盖所有奖励簇，同时保持较高的平均奖励。}
    \label{fig:toy_experiment}
    \vspace{-1.5em}
\end{figure}

% ---- P1: 大背景 + gap ----
近期，强化学习已经在LLM和生成式diffusion和flow-matching模型的对齐上取得了显著的成功，但现有的方法在训练的时候会产生reward hacking，也就是模型学会利用奖励函数或奖励模型的缺陷，通过过度强化少数高奖励的模型来提高奖励分数，进而导致mode collapse。缓解reward hacking的问题在LLM领域已经有充分的探索，但是在生成diffusion模型方面对此的探索明显不足(remains largely unexplored)。这个问题对于生成模型而言更为迫切，因为reward hacking会导致：(1).多样性的丧失：对于语言模型而言，问题可能有唯一确定的答案，但是对于生成模型例如文生图模型而言，同一个prompt可以对应很多在composition、spatial layout和场景语义（如figure1）上多样的可行结果，而reward hacking会让生成模型的结果只探索到几个固定的构图和风格，如图xxx (2).不可靠奖励信号的放大：对于文生图模型，无论是基于模型的奖励（例如ImageReward~\cite{xu2023imagereward}、HPS~\cite{wu2023hpsv2}、PickScore~\cite{kirstain2023pick}），还是基于规则的奖励（例如OCR 准确率、GenEval~\cite{ghosh2024geneval}），本质上是人类偏好的不完美代理。~\cite{gao2023scaling,chen2023textdiffuser}，~\cite{pan2022the,skalse2022defining,he2025gardo}，在这些代理奖励上的reward hacking会放大那些被奖励模型误判为高质量、但并不真正符合人类偏好的图像属性，从而导致生成质量下降。所以这就引出了生成模型对齐的核心问题：\textit{如何在保留生成式扩散模型从预训练数据学习到的各向异性的生成结果的分布的同时，让模型尽可能去迎合有特定偏好的奖励？}

% ---- P2: 根因分析（mode-seeking）+ 核心洞察（mode-covering）----
生成式diffusion和flow-matching模型的reward hacking行为can be attributed to当前diffusion-based RL的训练目标的问题。当前方法以最大化奖励作为优化目标~\cite{DDPO,fan2023dpok,liu2025flowgrpo,xue2025dancegrpo,li2025mixgrpo,ding2026treegrpo}，which被我们证明内在上(intrinstic)是\textit{模式寻求（mode-seeking）}的，也就是说模型倾向于生成最容易拿到high reward的一类结果，也不愿覆盖所有可能的合理结果，如图()中GRPO的例子所示。理想中的优化目标应该是mode-covering的，也就是说模型不只追求最高分结果，而是尽量覆盖所有合理解，。这一分析进一步表明，缓解reward hacking需要从根本上改变优化目标。existing工作主要通过两条路径来尝试解决这个问题：（1）约束过度优化：通过KL正则化~\cite{ouyang2022training,stiennon2020learning,fan2023dpok,liu2025flowgrpo,he2025gardo}来限制策略相较于参考模型的偏移，但是并没有改变算法最大化奖励的优化目标，生成结果的多样性改善有限；（2）改进训练目标：通过GFlowNet-based方法~\cite{zhang2024dgfs,zhang2025improving,liu2025nablagfn}来让生成结果的概率与奖励成比例，但现有形式通常只在单个去噪步骤上建立局部约束，需要估计一个无法求解的state flow 函数来逐步回传reward信号进行更新，从而引入额外的训练误差。因此，我们的核心洞察是：\textbf{Diffusion-based RL的优化目标不应该是最大化奖励，而应该在完整去噪轨迹-level让生成路径的概率匹配奖励分布。}

% ---- P3: 方法——Softmax-TB 目标 ----
基于这一洞察，我们提出\textbf{轨迹匹配策略优化（TMPO）}，将优化目标从奖励最大化变为轨迹级别上的reward distributon matching。我们证明TMPO是mode-covering的，可以天然的鼓励合理解的覆盖，从而从根本上缓解reward hacking问题，如图~\ref{fig:toy_experiment}所示。Specifically,我们introduce\textbf{Softmax 轨迹平衡（Softmax-TB）}——一个无需配分函数的轨迹级分布匹配目标。对于从同一个起点产生的 $K$ 条轨迹，TMPO 将这些轨迹的生成概率与一个由奖励计算得到的 Boltzmann 目标分布进行匹配： $p^*(\tau) \propto \exp(\beta R(\tau))$，让高奖励的结果可以获得相对较高的生成概率（？）。同时，我们通过对组内 $K$ 条轨迹概率奖励和奖励进行归一化，消除了无法计算的配分函数。为了降低sotmax-TB需要完整采样多个轨迹导致的训练时间开销~\cite{zhang2025improving}，TMPO 进一步引入\textbf{动态前缀共享树采样器}~\cite{li2025mixgrpo,fu2025dynamictreerpo,ding2026treegrpo}，让 $K$ 条轨迹通过树状结构共享部分去噪步骤，减少了重复计算，大幅降低了训练时间开销，并通过动态调整树状分支点，鼓励模型在去噪的不同阶段进行有效的探索，提升了训练的效果。

% ---- P5: 实验结果 ----
我们在 FLUX.1-dev 上跨人类偏好、组合生成和文字渲染三类对齐任务评估 TMPO。结果表明，TMPO 在所有设置下均实现了最优的奖励-多样性权衡：生成多样性（LGMD 和余弦多样性）相比当前最优方法提升 9.1\%，在 GenEval 和 PickScore 上取得最高任务奖励，OCR 上保持竞争力，每次迭代训练时间相比SOTA方法减少最多 27\%，并在所有基线中主导奖励-多样性和奖励-efficiency的 Pareto 前沿（图~\ref{fig:pareto}）。

% ---- P6: 贡献总结 ----
我们的贡献如下：（1）我们揭示奖励最大化的优化目标是扩散 RL 多样性崩塌的根因，并将优化目标转换为在完整去噪轨迹上的奖励分布匹配。（2）我们引入了\textbf{Softmax 轨迹平衡}，一个无需配分函数的轨迹平衡目标，并证明其模式覆盖性质可以天然保持分布多样性。（3）我们引入动态前缀共享树采样器，大幅降低了轨迹平衡目标的训练时间，实现在大规模流匹配模型上的可扩展训练。


==> NeurIPS_2026_TMPO__Preprint_/sections/method.tex <==
\section{Trajectory Matching Policy Optimization}
\label{headings}

In this section, we present \textbf{Trajectory Matching Policy Optimization (TMPO)} for online reward-induced trajectory distribution matching in flow-matching text-to-image models. We adapt GFlowNet trajectory balance to within-prompt trajectory groups, yielding a partition-free \textbf{Softmax-TB} objective with provable mode-covering properties (Section~\ref{prop:mode_covering}). We then describe how reward-bearing samples are efficiently collected through prefix-sharing SDE tree rollouts with \textbf{Dynamic Stochastic Tree Sampling}. The overall pipeline is illustrated in Figure~\ref{fig:pipeline}.

\begin{figure*}[ht]
  \centering
  \includegraphics[width=\textwidth]{figures/TMPO.pdf}
  \caption{\textbf{Overview of the TMPO framework.} For each prompt, Dynamic Stochastic Tree Sampling shares a deterministic ODE prefix and injects SDE noise at three curriculum-scheduled branch points, yielding $3^3{=}27$ trajectories with reduced compute. Terminal images are scored by a reward model, and Softmax Trajectory Balance converts the rewards into a Boltzmann target, computing the per-trajectory advantage as the log-ratio between the target and policy distributions.}
  \label{fig:pipeline}
  \vspace{-1.5em}
\end{figure*}

\subsection{From GFlowNets to Softmax Trajectory Balance}

GFlowNets learn a policy $\pi_\theta$ such that $P_\theta(\tau) \propto R(\tau)$ by minimizing a trajectory balance (TB) residual:
\begin{equation}
    \mathcal{L}_{\text{TB}}(\tau) = \bigl( \log Z + \log P_{\theta}(\tau) - \log R(\tau) \bigr)^2,
\end{equation}
where $Z$ is the partition function typically estimated via an auxiliary network. In TMPO's tree topology, all $K$ trajectories for the same prompt share a common $Z$, so normalizing within the group cancels the partition function exactly: $P_\theta(\tau_i)/\sum_j P_\theta(\tau_j) = R(\tau_i)/\sum_j R(\tau_j)$ (Appendix~\ref{appendix:theoretical_derivations}).

To introduce adjustable sharpness, we replace raw rewards with a Boltzmann target $p^*(\tau) \propto \exp(\beta R(\tau))$, where $\beta$ controls mode concentration. This is the maximum-entropy distribution subject to the expected reward constraint (Appendix~\ref{appendix:theoretical_derivations}). Substituting into the within-group matching and defining shorthand $q_i \triangleq \mathrm{softmax}_i(\beta R)$ and $p_i \triangleq P_\theta(\tau_i)/\sum_j P_\theta(\tau_j)$, we obtain the \textbf{Softmax-TB advantage}:
\begin{equation}
    A_i = \log q_i - \log p_i = \log \frac{\exp(\beta R_i)}{\sum_{j=1}^K \exp(\beta R_j)} - \log \frac{P_{\theta}(\tau_i)}{\sum_{j=1}^K P_{\theta}(\tau_j)}
\end{equation}
The following result shows that the Softmax-TB advantage is intimately connected to forward KL minimization.

\paragraph{Mode-Covering Equilibrium.}\label{prop:mode_covering}
Let $q_i = \exp(\beta R_i)/\sum_{j=1}^K \exp(\beta R_j)$ denote the within-group Boltzmann target and $p_i = P_\theta(\tau_i)/\sum_{j=1}^K P_\theta(\tau_j)$ the within-group policy distribution. Then the Boltzmann-weighted Softmax-TB advantage equals the within-group forward KL divergence:
\[
\sum_{i=1}^K q_i \, A_i = D_{\mathrm{KL}}^{(K)}(q_\beta \,\|\, p_\theta) \;\geq\; 0,
\]
with equality if and only if $p_i = q_i$ for all $i$. Because $D_{\mathrm{KL}}^{(K)}(q \| p) \to +\infty$ whenever $p_i \to 0$ for any $i$ with $q_i > 0$, Softmax-TB inherently penalizes under-coverage of any mode that carries positive Boltzmann weight. Within-group normalization cancels $Z_\beta$ and $Z_\theta$, making this conditional forward KL exactly computable over the $K$ observed trajectories, without requiring independent samples from the global intractable $q_\beta$ (extended proof and quantitative bounds in Appendix~\ref{appendix:forward_kl}).

\textit{Proof.} By definition, $A_i = \log q_i - \log p_i$. Substituting into the Boltzmann-weighted sum: $\sum_i q_i A_i = \sum_i q_i (\log q_i - \log p_i) = D_{\mathrm{KL}}^{(K)}(q \| p)$. Non-negativity and the equality condition follow from Gibbs' inequality. Since both $q$ and $p$ are normalized within the group, the global partition function $Z_\beta$ and the policy's total probability $Z_\theta$ cancel and need not be estimated. \hfill$\square$

\paragraph{Reverse KL vs.\ Forward KL.}\label{remark:mode_seeking}
Standard policy gradient methods sample from $\pi_\theta$ and therefore exhibit reverse-KL-like, mode-seeking behavior: under the entropy-regularized Boltzmann formulation, reward maximization (e.g., Flow-GRPO, TreeGRPO) can be interpreted as minimizing $D_{\mathrm{KL}}(p_\theta \| q_\beta)$ (Appendix~\ref{appendix:reverse_kl_comparison}). Its advantage $A_i \propto R_i - \bar{R}$ is agnostic to the policy probability $p_i$, so dropping a mode incurs no direct gradient penalty. In contrast, TMPO's log-ratio advantage $A_i = \log(q_i/p_i)$ is distribution-aware: it diverges whenever any mode with positive Boltzmann weight is under-covered ($p_i \to 0 \Rightarrow A_i \to +\infty$), inheriting the mode-covering behavior of forward KL despite sampling from the policy. \textbf{This distinction---the distribution-aware advantage of Equation~\eqref{eq:advantage}---provides the theoretical basis for diversity preservation without auxiliary KL regularization.}

\paragraph{Complete Softmax-TB Objective}
Since $A_i$ involves the shared softmax denominator that couples all $K$ trajectories, we detach it as a stop-gradient signal and route the gradient exclusively through the IS ratio $\hat{\rho}_i$. The complete TMPO loss is:
\begin{gather}
\boxed{
\mathcal{L}_{\text{TMPO}} = -\frac{1}{K}\sum_{i=1}^{K} \min\!\Bigl(\hat{\rho}_i \, A_i^{\bot},\;\operatorname{clip}\!\bigl(\hat{\rho}_i,\;1{-}\varepsilon,\;1{+}\varepsilon\bigr)\, A_i^{\bot}\Bigr)
} \label{eq:softmax_tb_loss} \\[4pt]
A_i = \log\frac{\exp(\beta R_i)}{\sum_{j=1}^K\exp(\beta R_j)} - \log\frac{P_\theta(\tau_i)}{\sum_{j=1}^K P_\theta(\tau_j)},\qquad \hat{\rho}_i = \prod_{t=1}^{T}\frac{\pi_\theta(x_{s_t^-}^{(i)} \mid x_{s_t}^{(i)})}{\pi_{\theta_{\text{old}}}(x_{s_t^-}^{(i)} \mid x_{s_t}^{(i)})} \label{eq:advantage}
\end{gather}
Here $A_i^{\bot}$ denotes the stop-gradient advantage and $\hat{\rho}_i$ is clipped to $[1{-}\varepsilon, 1{+}\varepsilon]$ for trust-region protection~\cite{schulman2017proximal}. The per-step log-ratios are centered via RatioNorm~\cite{wang2025grpo} to remove the deterministic negative shift of Gaussian transition kernels and restore symmetric clipping (Appendix~\ref{appendix:gradient_analysis}).

\subsection{Dynamic Stochastic Tree Sampling}
\label{sec:tree_sampling}

Unlike the independent parallel rollouts in standard GRPO-based methods~\cite{liu2025flowgrpo,xue2025dancegrpo}, TMPO places three consecutive stochastic branch points along the denoising trajectory, producing a $3^3{=}27$ terminal tree per prompt. At each branch point, $B{=}3$ child trajectories are spawned from independent noise realizations. Early branch points at high noise levels introduce coarse-grained diversity across trajectory groups, while later branch points at lower noise levels supply finer-grained structured variations. Shared prefix computations before each bifurcation substantially reduce the cost of RL training on large-scale models such as FLUX.

\paragraph{Dynamic Branching Schedule}
Branch positions follow a curriculum that shifts from early high-noise regions toward later structured regions as training progresses ($p = \mathrm{clip}(u/U, 0, 1)$). To prevent overfitting to a fixed tree geometry, each position is stochastically perturbed:
\begin{equation}
\xi_i \sim \mathrm{Beta}(\kappa \bar{\mu}_i(p),\, \kappa(1{-}\bar{\mu}_i(p))), \quad \tilde{s}_i = \lfloor s_{\min} + (s_{\max} - s_{\min})\xi_i + 0.5 \rfloor
\end{equation}
with final indices obtained by sorting. At each branch point $s_i$, child nodes are generated by injecting SDE noise with magnitude $\gamma(\sigma) = \eta\sqrt{\sigma/(1{-}\sigma)}\sqrt{-\Delta t}$, where $\eta{=}0.7$ following the CPS recommendation~\cite{wang2025cps}:
\begin{equation}
x_{s_i^-}^{(r)} = \mu_{\theta}(x_{s_i}, s_i) + \gamma(\sigma_{s_i})\varepsilon_r, \quad \varepsilon_r \sim \mathcal{N}(0, \mathbf{I})
\end{equation}
Between branch points, the denoising trajectory follows deterministic ODE steps that do not require gradient computation. The trajectory log-probability accumulates only the $T$ stochastic transitions at branch points: $\log P_\theta(\tau) = \sum_{i=1}^{T} \log \pi_\theta(x_{s_i^-} \mid x_{s_i})$, so gradient back-propagation is confined to $T$ steps rather than the full denoising horizon, substantially reducing per-iteration training cost. Full derivations of the SDE noise injection, Beta branching schedule, and log-probability computation are provided in Appendix~\ref{appendix:tree_sampling}.


==> NeurIPS_2026_TMPO__Preprint_/sections/method_zh.tex <==
\section{轨迹匹配策略优化}
\label{headings}

在本节中，我们提出\textbf{轨迹匹配策略优化（Trajectory Matching Policy Optimization, TMPO）}，用于流匹配文生图模型中的在线奖励引导轨迹分布匹配。我们将GFlowNet的轨迹平衡适配到同一提示词的轨迹组内，得到一个无需分区函数的\textbf{Softmax-TB}目标函数，并具有可证明的模式覆盖性质（命题~\ref{prop:mode_covering}）。随后，我们描述如何通过前缀共享的SDE树状展开，结合\textbf{动态随机树采样}高效收集含奖励的样本。整体流程如图~\ref{fig:pipeline}所示。

\begin{figure*}[ht]
  \centering
  \includegraphics[width=\textwidth]{figures/TMPO.pdf}
  \caption{TMPO框架概览。对于每个提示词，动态随机树采样共享一段确定性ODE前缀，并在三个课程调度的分支点注入SDE噪声，以较低的计算开销生成$3^3{=}27$条轨迹。终端图像由奖励模型评分，Softmax轨迹平衡将奖励转化为Boltzmann目标分布，计算每条轨迹的优势值为目标分布与策略分布的对数比。}
  \label{fig:pipeline}
\end{figure*}

\subsection{从GFlowNets到Softmax轨迹平衡}

GFlowNets学习一个策略$\pi_\theta$使得$P_\theta(\tau) \propto R(\tau)$，通过最小化轨迹平衡（TB）残差实现：
\begin{equation}
    \mathcal{L}_{\text{TB}}(\tau) = \bigl( \log Z + \log P_{\theta}(\tau) - \log R(\tau) \bigr)^2,
\end{equation}
其中$Z$是通常通过辅助网络估计的分区函数。在TMPO的树状拓扑中，反向路径概率$P_B(\tau_i) = 1$，平衡条件简化为$P_\theta(\tau_i) = R(\tau_i) / Z$。关键在于，由于同一提示词生成的所有$K$条轨迹共享相同的$Z$，在组内归一化可以精确消去分区函数：$P_\theta(\tau_i)/\sum_j P_\theta(\tau_j) = R(\tau_i)/\sum_j R(\tau_j)$（附录~\ref{appendix:theoretical_derivations}）。

为引入可调的锐度，我们将原始奖励替换为Boltzmann目标分布$p^*(\tau) \propto \exp(\beta R(\tau))$，其中$\beta$控制模式集中程度。这是在期望奖励约束下的最大熵分布（附录~\ref{appendix:theoretical_derivations}）。将其代入组内匹配并定义简记$q_i \triangleq \mathrm{softmax}_i(\beta R)$和$p_i \triangleq P_\theta(\tau_i)/\sum_j P_\theta(\tau_j)$，我们得到\textbf{Softmax-TB优势}：
\begin{equation}
    A_i = \log q_i - \log p_i = \log \frac{\exp(\beta R_i)}{\sum_{j=1}^K \exp(\beta R_j)} - \log \frac{P_{\theta}(\tau_i)}{\sum_{j=1}^K P_{\theta}(\tau_j)}
\end{equation}
对数比$A_i = \log(q_i/p_i)$是\emph{分布感知的}：当任何具有正Boltzmann权重的模式被欠覆盖时（$p_i \to 0$），它趋向发散（$A_i \to +\infty$），提供了仅基于奖励的优势中所缺失的内在防坍缩信号。以下命题形式化了这一联系。

\begin{proposition}[模式覆盖均衡]\label{prop:mode_covering}
令$q_i = \exp(\beta R_i)/\sum_{j=1}^K \exp(\beta R_j)$为组内Boltzmann目标分布，$p_i = P_\theta(\tau_i)/\sum_{j=1}^K P_\theta(\tau_j)$为组内策略分布。则Boltzmann加权的Softmax-TB优势等于组内前向KL散度：
\[
\sum_{i=1}^K q_i \, A_i = D_{\mathrm{KL}}^{(K)}(q_\beta \,\|\, p_\theta) \;\geq\; 0,
\]
当且仅当$p_i = q_i$对所有$i$成立时等号成立，其中上标$(K)$强调该散度是在每个提示词特定组内的$K$个离散原子上计算的。由于当$q_i > 0$的任意$i$满足$p_i \to 0$时$D_{\mathrm{KL}}^{(K)}(q \| p) \to +\infty$，Softmax-TB本质上惩罚对任何具有正Boltzmann权重的模式的欠覆盖。关键的是，组内归一化使得这一前向KL可以在$K$条观测轨迹上精确计算，而无需从难以处理的Boltzmann目标$q_\beta$中采样。
\end{proposition}
\begin{proof}
根据定义，$A_i = \log q_i - \log p_i$。代入Boltzmann加权求和：$\sum_i q_i A_i = \sum_i q_i (\log q_i - \log p_i) = D_{\mathrm{KL}}^{(K)}(q \| p)$。非负性和等号条件由Gibbs不等式得出。由于$q$和$p$均在组内归一化，全局分区函数$Z_\beta$和策略的总概率$Z_\theta$相消，无需估计。
\end{proof}

\begin{remark}\label{remark:mode_seeking}
所有策略梯度方法从$\pi_\theta$采样，因此自然处于反向KL体制下：标准的奖励最大化方法（如FlowGRPO、TreeGRPO）可以被证明隐式最小化$D_{\mathrm{KL}}(p_\theta \| q_\beta)$（附录~\ref{appendix:reverse_kl_comparison}），其优势$A_i \propto R_i - \bar{R}$与策略概率$p_i$无关；丢弃一个模式不产生梯度惩罚。相比之下，TMPO的对数比优势$A_i = \log(q_i/p_i)$是分布感知的：当任何具有正Boltzmann权重的模式被欠覆盖时它趋向发散（$p_i \to 0 \Rightarrow A_i \to +\infty$），尽管从策略采样，仍继承了前向KL的模式覆盖渐近行为。我们注意到这是在$K$条观测轨迹上的\emph{组内}性质，而非全局分布保证；然而，它提供了比GRPO的纯奖励优势更严格的多样性信号，后者对丢弃的模式不产生梯度惩罚。\textbf{这一结构性区别，而非采样分布本身，为无需辅助KL正则化的多样性保持提供了理论基础。}
\end{remark}

\paragraph{完整的Softmax-TB目标函数}
由于$A_i$涉及耦合所有$K$条轨迹的共享softmax分母，我们将其作为止梯度信号分离，梯度仅通过重要性采样比$\hat{\rho}_i$传播。完整的TMPO损失为：
\begin{gather}
\boxed{
\mathcal{L}_{\text{TMPO}} = -\frac{1}{K}\sum_{i=1}^{K} \min\!\Bigl(\hat{\rho}_i \, A_i^{\bot},\;\operatorname{clip}\!\bigl(\hat{\rho}_i,\;1{-}\varepsilon,\;1{+}\varepsilon\bigr)\, A_i^{\bot}\Bigr)
} \label{eq:softmax_tb_loss} \\[4pt]
A_i = \log\frac{\exp(\beta R_i)}{\sum_{j=1}^K\exp(\beta R_j)} - \log\frac{P_\theta(\tau_i)}{\sum_{j=1}^K P_\theta(\tau_j)},\qquad \hat{\rho}_i = \prod_{t=1}^{T}\frac{\pi_\theta(x_{s_t^-}^{(i)} \mid x_{s_t}^{(i)})}{\pi_{\theta_{\text{old}}}(x_{s_t^-}^{(i)} \mid x_{s_t}^{(i)})} \label{eq:advantage}
\end{gather}
其中$A_i^{\bot}$为止梯度优势，$\beta$为逆温度，$\varepsilon$为裁剪半径，$\hat{\rho}_i = \prod_t (\pi_\theta / \pi_{\theta_{\text{old}}})$为轨迹级重要性采样比，裁剪至$[1{-}\varepsilon, 1{+}\varepsilon]$以实现信任域保护~\cite{schulman2017proximal}。实践中，逐步对数比通过RatioNorm~\cite{wang2025grpo}进行中心化，以消除高斯转移核的确定性负偏移并恢复对称裁剪（附录~\ref{appendix:gradient_analysis}）。

\subsection{动态随机树采样}
\label{sec:tree_sampling}

与标准GRPO类方法中的独立并行展开不同~\cite{liu2025flowgrpo,xue2025dancegrpo}，TMPO沿去噪轨迹设置三个连续的随机分支点。在每个分支点，采样器注入三个独立的SDE噪声实现，每个提示词生成一棵$3^3{=}27$的终端树。每次分叉前的共享前缀计算大幅降低了在FLUX等大规模模型上进行强化学习训练的开销，同时为Softmax-TB提供了结构化的组内多样性。

\paragraph{动态分支调度}
分支位置由一个课程调度器控制，该调度器以归一化训练进度$p = \mathrm{clip}(u/U, 0, 1)$为参数。随着训练推进，均值位置$\bar{\mu}_i(p)$从早期的高噪声区域向后期的结构化去噪区域移动。为防止对固定树结构的过拟合，每个位置经过随机扰动：
\begin{equation}
\xi_i \sim \mathrm{Beta}(\kappa \bar{\mu}_i(p),\, \kappa(1{-}\bar{\mu}_i(p))), \quad \tilde{s}_i = \lfloor s_{\min} + (s_{\max} - s_{\min})\xi_i + 0.5 \rfloor
\end{equation}
最终索引通过排序获得。在每个分支点$s_i$处，子节点通过注入幅度为$\gamma_i(\sigma) = \eta_i\sqrt{\sigma/(1{-}\sigma)}\sqrt{-\Delta t}$的SDE噪声生成：
\begin{equation}
x_{s_i^-}^{(r)} = \mu_{\theta}(x_{s_i}, s_i) + \gamma_i(\sigma_{s_i})\varepsilon_r, \quad \varepsilon_r \sim \mathcal{N}(0, \mathbf{I})
\end{equation}
分支点之间，去噪轨迹遵循不需要梯度计算的确定性ODE步骤。轨迹对数概率仅在$T$个分支点的随机转换处累积：$\log P_\theta(\tau) = \sum_{i=1}^{T} \log \pi_\theta(x_{s_i^-} \mid x_{s_i})$，因此梯度反向传播仅限于$T$步而非完整的去噪时间跨度，大幅降低了每次迭代的训练开销。SDE噪声注入、Beta分支调度和对数概率计算的完整推导见附录~\ref{appendix:tree_sampling}。


==> NeurIPS_2026_TMPO__Preprint_/sections/preliminaries.tex <==
\iffalse
\section{Preliminaries}
\label{gen_inst}
\subsection{Trajectory Balance in GFlowNets}

Let $\mathcal{X}$ denote a set of combinatorial objects, and let $R$ be a reward function that assigns a non-negative value to each object $x \in \mathcal{X}$. GFlowNets learn a sequential constructive policy $\pi$ such that the probability of generating an object $x$ is proportional to its reward, that is, $\pi(x) \propto R(x)$.

This generation process can be represented by a directed acyclic graph (DAG) $G = (\mathcal{S}, \mathcal{A})$, where each vertex $s \in \mathcal{S}$ denotes a state and each directed edge $(u \to v) \in \mathcal{A}$ denotes an action. Generating an object $x \in \mathcal{X}$ corresponds to a complete trajectory $\tau = (s_{0}\to \dots \to s_{n}) \in \mathcal{T}$ in the DAG, which starts from the initial state $s_{0}$ and ends at a terminal state $s_n \in \mathcal{X}$.

The state flow $F(s)$ is a non-negative weight associated with each state $s \in \mathcal{S}$. The forward policy $P_F(s' \mid s)$ specifies the probability of transitioning to a child state $s'$, whereas the backward policy $P_B(s \mid s')$ specifies the probability of transitioning to the parent state $s$. Detailed balance enforces local flow consistency along every edge $(s \to s') \in \mathcal{A}$:
\begin{equation}
    \forall(s \to s') \in \mathcal{A}, \quad F_{\theta}(s) P_{F}(s' \mid s; \theta) = F_{\theta}(s') P_{B}(s \mid s'; \theta).
\end{equation}

To enforce this consistency, GFlowNets use training objectives at different granularities, including detailed balance, trajectory balance, and sub-trajectory balance. Because these objectives are diversity seeking by design, GFlowNets have been applied successfully to molecular generation, diffusion-model fine-tuning, and amortized inference.

Among these objectives, trajectory balance enforces global consistency at the trajectory level and is defined as
\begin{equation}
    Z_{\theta}\prod_{t=1}^{n}P_{F}(s_{t}\mid s_{t-1}; \theta) = R(x) \prod_{t=1}^{n}P_{B}(s_{t-1}\mid s_{t}; \theta).
\end{equation}

\subsection{RL for Diffusion and Flow Models}

The generation process of a diffusion model can be formulated as a Markov decision process (MDP) with $T$ discrete time steps. In this setting, the state $s_t$ corresponds to the latent variable $x_t$ at diffusion step $t$, and the action $a_t$ corresponds to the transition from $x_t$ to $x_{t-\Delta t}$. RL fine-tuning optimizes the policy $\pi_{\theta}(x_{t-\Delta t} \mid x_t)$ of a pretrained model so as to maximize the expected reward $R(x_0)$ of the final generated sample $x_0$.

\paragraph{Flow matching and rectified flow}
This paper focuses on flow-matching models such as Flux. Rectified Flow (RF) defines a linearly interpolated probability flow:
\begin{equation}
    x_t = t x_1 + (1-t) x_0, \quad t \in [0, 1]
\end{equation}
where $x_1 \sim \mathcal{N}(0, \mathbf{I})$ is Gaussian noise and $x_0$ is the target sample. Training aims to predict the velocity field $v_{\theta}(x_t, t) = \frac{dx_t}{dt}$. During sampling, generation from noise to data is obtained by solving the following ODE:
\begin{equation}
    dx_t = v_{\theta}(x_t, t) \, dt.
\end{equation}

\paragraph{Stochastic exploration and log-probability}
To enable exploration in RL, the deterministic ODE is commonly converted into an equivalent stochastic differential equation (SDE):
\begin{equation}
    dx_t = [v_{\theta}(x_t, t) + f(x_t, t)] \, dt + g(t) \, dw
\end{equation}
where $dw$ is a standard Wiener process and $f(x_t, t)$ is a correction term. In discrete-time sampling, the transition probability from $x_t$ to $x_{t-\Delta t}$ follows a Gaussian distribution, $\pi_{\theta}(x_{t-\Delta t} \mid x_t) = \mathcal{N}(\mu_{\theta}, \sigma_t^2 \Delta t)$. The corresponding one-step log-probability is
\begin{equation}
    \log \pi_{\theta}(x_{t-\Delta t} \mid x_t) = -\frac{\|x_{t-\Delta t} - \mu_{\theta}\|^2}{2\sigma_t^2 \Delta t} - \frac{d}{2}\log(2\pi \sigma_t^2 \Delta t).
\end{equation}
Conventional diffusion-RL methods such as PPO and GRPO use this log-probability to compute policy gradients and update model parameters through importance sampling so that generated trajectories move toward the preference distribution defined by a reward model.
\fi

\section{Preliminaries}
\label{gen_inst}

\subsection{Trajectory Balance and Reward Matching}

Generative Flow Networks (GFlowNets) train stochastic policies to sample terminal objects in proportion to non-negative rewards~\cite{bengio2021flow}. For a trajectory $\tau=(s_0\to\cdots\to s_n)$ ending at $x=s_n$ with reward $R(x)$, Trajectory Balance (TB) imposes:~\cite{malkin2022trajectory}

\begin{equation}
    Z_{\theta}\prod_{t=1}^{n}P_F(s_t\mid s_{t-1};\theta)
    =
    R(x)\prod_{t=1}^{n}P_B(s_{t-1}\mid s_t;\theta),
    \label{eq:prelim_tb}
\end{equation}
where $P_F$, $P_B$, and $Z_\theta$ are the forward policy, backward policy, and total flow. This reward-proportional view preserves multiple high-reward modes. Diffusion GFlowNet methods and Flow-GRPO similarly motivate replacing scalar reward maximization with reward distribution matching~\cite{zhang2024dgfs,liu2025nablagfn,zhu2025flowrl}.

\subsection{ODE-to-SDE Conversion for Stochastic Diffusion Policies}

Modern text-to-image generators are commonly built on diffusion or flow-matching models~\cite{ho2020denoising,rombach2022high,lipman2023flow,liu2023flow,albergo2023stochastic,esser2024scaling,flux2024}. In rectified flow, a clean sample $x_0$ and noise $x_1\sim\mathcal{N}(0,\mathbf{I})$ are connected by:
\begin{equation}
    x_t=(1-t)x_0+t x_1,\qquad
    d x_t=v_{\theta}(x_t,t,c)\,dt ,
    \label{eq:prelim_rf}
\end{equation}
Deterministic ODE solvers~\cite{song2021denoising,lu2022dpmsolver} lack the transition probabilities required by policy-gradient RL. Following prior work~\cite{song2020score,liu2025flowgrpo,xue2025dancegrpo}, we convert the probability-flow ODE to an equivalent SDE that admits tractable likelihoods for credit assignment while preserving marginals:
\begin{equation}
    d x_t =
    \left[
        v_{\theta}(x_t,t,c)
        + \frac{1}{2}\sigma^2(t)\nabla_{x}\log p_{\theta}(x_t\mid c,t)
    \right]dt
    + \sigma(t)dW_t .
    \label{eq:prelim_probability_flow_sde}
\end{equation}
Here $\sigma(t)$ controls the noise scale, with $\sigma(t)\equiv 0$ recovering the deterministic ODE.


==> NeurIPS_2026_TMPO__Preprint_/sections/related_work.tex <==
\section{Related Work}

\paragraph{Mitigating reward hacking in diffusion model alignment.}
Diffusion-based RL alignment is highly susceptible to reward hacking under model-based or rule-based rewards~\cite{pan2022the,skalse2022defining,hong2026understanding,wu2025rewarddance}. Existing mitigations, including KL regularization~\cite{fan2023dpok,liu2025flowgrpo}, pairwise preference rewards~\cite{wang2025pref}, and diversity-aware regularization~\cite{he2025gardo}, still optimize scalar rewards and thus inherit mode-collapse risks~\cite{gx2025kl}. TMPO addresses this limitation by reformulating scalar rewards as a preference distribution to be matched.

\paragraph{Distribution matching and GFlowNet-based alignment.}
GFlowNets train stochastic policies with terminal distributions proportional to rewards~\cite{bengio2021flow}. DGFS~\cite{zhang2024dgfs}, DAG~\cite{zhang2025improving}, and $\nabla$-GFlowNet~\cite{liu2025nablagfn} adapt this idea to diffusion alignment using local detailed-balance objectives, with $\nabla$-GFlowNet further incorporating reward gradients. However, their local or partial-trajectory constraints require intractable state-flow estimation and can accumulate errors over long denoising horizons. TMPO instead directly matches complete trajectory probabilities to a reward-induced Boltzmann distribution, avoiding per-transition flow estimation and explicit partition computation.

\paragraph{Efficient trajectory sampling in diffusion model alignment.}
RL post-training for large-scale flow models is bottlenecked by redundant rollouts, and complete-trajectory objectives amplify this cost by requiring policy probabilities over multiple trajectories~\cite{zhang2025improving}. MixGRPO reduces stochastic optimization to selected SDE windows~\cite{li2025mixgrpo}, while Dynamic-TreeRPO and TreeGRPO amortize early computation by sharing denoising prefixes~\cite{fu2025dynamictreerpo,ding2026treegrpo}. TMPO adopts prefix sharing and further introduces dynamic branching schedules to maintain effective exploration across training stages.

==> NeurIPS_2026_TMPO__Preprint_/sections/teaser.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]{figures/1_comparison.pdf}
    \caption{\textbf{Generative diversity comparison between TMPO (Ours) and Flow-GRPO.}}
    \label{fig:comparison}
\end{figure}


==> NeurIPS_2026_TMPO__Preprint_/template/dark.tex <==

\usepackage{xcolor}
\definecolor{coolblack}{RGB}{40, 40, 45}
\definecolor{coolwhite}{RGB}{160, 160, 160}
\definecolor{coolblue}{RGB}{65, 130, 205}
\pagecolor{coolblack}
\color{coolwhite}   
\PassOptionsToPackage{allbordercolors=coolblue,allcolors=coolblue,colorlinks=true}{hyperref}
\definecolor{coolred}{RGB}{200, 60, 100}
\renewcommand\note[1]{{\color{coolred} #1}}


==> NeurIPS_2026_TMPO__Preprint_/template/package.tex <==
%%%% Packages

%% Encoding
\usepackage{iftex}
\ifPDFTeX
  \usepackage[T1]{fontenc}
  \usepackage[utf8]{inputenc}
\fi
\usepackage[english]{babel}

%% Fonts — skip when fairmeta supplies its own
\makeatletter
\@ifclassloaded{fairmeta}{}{%
  \usepackage{times}
}
\makeatother

%% Links
\PassOptionsToPackage{hyphens}{url}
\usepackage{url}
\usepackage{hyperref}

%% Graphics
\usepackage{graphicx}
\usepackage{caption}
\makeatletter
\@ifclassloaded{fairmeta}{}{%
  \captionsetup{margin=10pt,font=small,labelfont=bf}
}
\makeatother
\usepackage{tikz}
\usetikzlibrary{positioning,shapes.geometric,calc}
\usepackage{pgfplots}
\pgfplotsset{compat=1.17}

%% Essentials

% Rendering enhancement
\usepackage{array}
\usepackage{booktabs}
\usepackage{microtype}
% Color
\usepackage{xcolor}
% Float
\usepackage{float}
% Itemize
\IfFileExists{enumitem.sty}{
  \usepackage{enumitem}
  \setitemize{itemsep=0pt,parsep=0pt,topsep=0pt}
  \setenumerate{itemsep=0pt,parsep=0pt,topsep=0pt}
}{}

% Algorithmic package
\IfFileExists{algorithm.sty}{
  \usepackage{algorithm}
  \usepackage{algorithmicx}
  \usepackage{algpseudocode}
}{}

%% Code listings (Lean 4)
\usepackage{listings}
\lstdefinestyle{lean}{
  basicstyle=\ttfamily\small,
  breaklines=true,
  columns=fullflexible,
  keepspaces=true,
  xleftmargin=4pt,
  aboveskip=6pt,
  belowskip=6pt,
  literate=
    {ℝ}{{$\mathbb{R}$}}1
    {ℕ}{{$\mathbb{N}$}}1
    {→}{{$\to$}}1
    {←}{{$\leftarrow$}}1
    {∀}{{$\forall$}}1
    {∃}{{$\exists$}}1
    {≤}{{$\le$}}1
    {≥}{{$\ge$}}1
    {≠}{{$\ne$}}1
    {⊆}{{$\subseteq$}}1
    {∈}{{$\in$}}1
    {∉}{{$\notin$}}1
    {⁻¹}{{$^{-1}$}}1
    {∫}{{$\int$}}1
    {α}{{$\alpha$}}1
    {·}{{$\cdot$}}1
    {⟩}{{$\rangle$}}1
    {⟨}{{$\langle$}}1
}
\lstset{style=lean}

%% Natbib bibliography
\usepackage{natbib}

%% To edit with several authors
\usepackage[normalem]{ulem}

% Bookcards

%% Per-book result cards (colored boxes in the per-book appendix)
\usepackage[most]{tcolorbox}
\newtcolorbox{bookcardbox}[1][]{%
  enhanced,
  breakable,
  colback=green!5!white,
  colframe=green!45!black,
  colbacktitle=green!18!white,
  coltitle=green!30!black,
  fonttitle=\bfseries,
  title filled,
  arc=6pt,
  boxrule=0.6pt,
  left=8pt,right=8pt,top=5pt,bottom=5pt,
  toptitle=3pt,bottomtitle=3pt,
  #1
}
% \bookcard{Title}{Author}{URL}{Targets}{Pages}{LoC}{Formalized}{Gaps}{Tokens}{Comments}
% (split in two stages because TeX macros are limited to 9 args)
\makeatletter
\newcommand{\bookcard}[2]{%
  \def\bk@title{#1}\def\bk@author{#2}\bookcard@aux
}
\newcommand{\bookcard@aux}[8]{%
  \begin{bookcardbox}[title={\emph{\bk@title}, by \bk@author}]
    \footnotesize
    \setlength{\extrarowheight}{2pt}%
    {\sloppy\raggedright\href{#1}{\nolinkurl{#1}}\par}\smallskip
    \begin{tabular}{@{}p{0.30\linewidth}p{0.36\linewidth}p{0.30\linewidth}@{}}
      \textbf{Target statements:} #2 &
      \textbf{Formalized statements:} #5 &
      \\
      \textbf{Pages:} #3 &
      \textbf{Lines of code:} #4 &
      \textbf{Tokens (M):} #7 \\
    \end{tabular}\par\smallskip
  \end{bookcardbox}%
}
\makeatother

